Presumptive Reasoning in a Paraconsistent Setting

We explore presumptive reasoning in the paraconsistent case. Specifically, we provide semantics for non-trivial reasoning with presumptive arguments with contradictory assumptions or conclusions. We adapt the case models proposed by Verheij and define the paraconsistent analogues of the three types of validity defined therein: coherent, presumptively valid, and conclusive ones. To formalise the reasoning, we define case models that use the expansion of the Belnap-Dunn logic with the Baaz Delta operator. We also show how to recover presumptive reasoning in the original, classical context from our paraconsistent version of case models. Finally, we construct a two-layered logic and obtain a faithful translation of presumptive arguments into formulas.

==> eptcsdata.tex <==
\providecommand{\firstpage}{233}
\providecommand{\publicationstatus}{R. Verbrugge (Ed.): Theoretical Aspects of \\
Rationality and Knowledge 2023 (TARK 2023)\\
EPTCS 379, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.379.19}{10.4204/EPTCS.379.19}}
\pdfoutput=1

